Trajectory-based Learning for Ball-in-Maze Games

Deep Reinforcement Learning has shown tremendous success in solving several games and tasks in robotics. However, unlike humans, it generally requires a lot of training instances. Trajectories imitating to solve the task at hand can help to increase sample-efficiency of deep RL methods. In this paper, we present a simple approach to use such trajectories, applied to the challenging Ball-in-Maze Games, recently introduced in the literature. We show that in spite of not using human-generated trajectories and just using the simulator as a model to generate a limited number of trajectories, we can get a speed-up of about 2-3x in the learning process. We also discuss some challenges we observed while using trajectory-based learning for very sparse reward functions.

==> egbib.tex <==
@inproceedings{mnih2016asynchronous,
  title={Asynchronous methods for deep reinforcement learning},
  author={Mnih, Volodymyr and Badia, Adria Puigdomenech and Mirza, Mehdi and Graves, Alex and Lillicrap, Timothy and Harley, Tim and Silver, David and Kavukcuoglu, Koray},
  booktitle={International conference on machine learning},
  pages={1928--1937},
  year={2016}
}
@inproceedings{nagabandi2018neural,
	title={Neural network dynamics for model-based deep reinforcement learning with model-free fine-tuning},
	author={Nagabandi, Anusha and Kahn, Gregory and Fearing, Ronald S and Levine, Sergey},
	booktitle={2018 IEEE International Conference on Robotics and Automation (ICRA)},
	pages={7559--7566},
	year={2018},
	organization={IEEE}
}
@inproceedings{ross2011reduction,
	title={A reduction of imitation learning and structured prediction to no-regret online learning},
	author={Ross, St{\'e}phane and Gordon, Geoffrey and Bagnell, Drew},
	booktitle={Proceedings of the fourteenth international conference on artificial intelligence and statistics},
	pages={627--635},
	year={2011}
}
